Fairness-aware Summarization for Justified Decision-Making

In consequential domains such as recidivism prediction, facility inspection, and benefit assignment, it's important for individuals to know the decision-relevant information for the model's prediction. In addition, predictions should be fair both in terms of the outcome and the justification of the outcome. In other words, decision-relevant features should provide sufficient information for the predicted outcome and should be independent of the membership of individuals in protected groups such as race and gender. In this work, we focus on the problem of (un)fairness in the justification of the text-based neural models. We tie the explanatory power of the model to fairness in the outcome and propose a fairness-aware summarization mechanism to detect and counteract the bias in such models. Given a potentially biased natural language explanation for a decision, we use a multi-task neural model and an attribution mechanism based on integrated gradients to extract high-utility and low-bias justifications in form of a summary. The extracted summary is then used for training a model to make decisions for individuals. Results on several real world datasets suggest that our method drastically limits the demographic leakage in the input (fairness in justification) while moderately enhancing the fairness in the outcome. Our model is also effective in detecting and counteracting several types of data poisoning attacks that synthesize race-coded reasoning or irrelevant justifications.

==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We discussed the limitations of our work at the end of Section~\ref{fairness-experimental-results}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Potential negative impacts of our proposed approach heavily are effected on how and where it is used.  While our model aims to avoid harms such as unfair justifications (e.g. arguments based on sex or race), one potential negative impact of our model is censorship of user reviews(e.g. if used for pre-processing or filtering what is presented on an online evaluation forum).}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We used publicly available datasets. See Section~\ref{fairly-justified-dataset} for more details. We will share our code online upon the acceptance of this work. }
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{fairness-training-details}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All the experiments are conducted 5 times and the results reflect average of all runs. We report the error bars in the supplementary material. }
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{fairness-training-details}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{We have included the URL to any assets we used. The license is shared in the corresponding web page for each asset.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We are planning to share our code upon acceptance of this work. }
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{For all our experiments we used publicly available data. }
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{The Rate My Professor dataset contains teaching evaluation for instructors. Often the name of the instructor is mentioned in the reviews. We anonymize this datasets by removing the names and pronouns from the reviews. See Section~\ref{fairly-justified-dataset} for more details.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> defs.tex <==
\newcommand{\moniba}[1]{\textcolor{purple}{\bf\small [#1 --MK]}}
\newcommand{\Moniba}[1]{\textcolor{purple}{\bf\small [#1 --MK]}}

\newcommand{\micha}[1]{\textcolor{green}{\bf\small [#1 --ME]}}
\newcommand{\Micha}[1]{\textcolor{green}{\bf\small [#1 --ME]}}

\newcommand{\Tanya}[1]{\textcolor{orange}{\bf\small [#1 --TB]}}
\newcommand{\tanya}[1]{\textcolor{orange}{\bf\small [#1 --TB]}}

\newcommand{\Srini}[1]{\textcolor{blue}{\bf\small [#1 --SP]}}
\newcommand{\srini}[1]{\textcolor{blue}{\bf\small [#1 --SP]}}


\newcommand{\removed}[1]{}
\newcommand{\REMOVED}[1]{}

\hyphenation{ana-lyze}
\hyphenation{ana-ly-sis}
\hyphenation{ana-ly-ses}


